Approximation and parameterized algorithms to find balanced connected partitions of graphs

Partitioning a connected graph into $k$~vertex-disjoint connected subgraphs of similar (or given) orders is a classical problem that has been intensively investigated since late seventies. Given a connected graph $G=(V,E)$ and a weight function $w : V \to \mathbb{Q}_\geq$, a connected $k$-partition of $G$ is a partition of $V$ such that each class induces a connected subgraph. The balanced connected $k$-partition problem consists in finding a connected $k$-partition in which every class has roughly the same weight. To model this concept of balance, one may seek connected $k$-partitions that either maximize the weight of a lightest class $(\text{max-min BCP}_k)$ or minimize the weight of a heaviest class $(\text{min-max BCP}_k)$. Such problems are equivalent when $k=2$, but they are different when $k\geq 3$. In this work, we propose a simple pseudo-polynomial $\frac{k}{2}$-approximation algorithm for $\text{min-max BCP}_k$ which runs in time $\mathcal{O}(W|V||E|)$, where $W = \sum_{v \in V} w(v)$. Based on this algorithm and using a scaling technique, we design a (polynomial) $(\frac{k}{2} +\varepsilon)$-approximation for the same problem with running-time $\mathcal{O}(|V|^3|E|/\varepsilon)$, for any fixed $\varepsilon>0$. Additionally, we propose a fixed-parameter tractable algorithm based on integer linear programming for the unweighted $\text{max-min BCP}_k$ parameterized by the size of a vertex cover.

==> Algorithms/max-min-alg.tex <==
\begin{algorithm}[H]
\hspace*{\algorithmicindent} \textbf{Input:} An instance~$(G, w)$ of~$\maxminBCP{4}$, where~$G$ is a~$2$-connected graph.\\
\hspace*{\algorithmicindent} \textbf{Output:} A connected~$3$-partition of~$G$.\\
\hspace*{\algorithmicindent} \textbf{Routine:} The algorithm~\textsc{Balance}~by Chleb{\'i}kov{\'a}~\cite{Chl96} to~$\maxminBCP{2}$. 
\begin{algorithmic}[1]
\Procedure {Balance3}{$G, w$}

\If {$\exists v^* \in V: w(v) \geq \frac{89}{400} W$}
	\State {\textbf{return} \textsc{Balance}($G - v^*, w$) $\cup~\{\{v^*\}\}$}
\Else
	\State {$Y \gets \{v^*\}$}
	\While {$w(Y) < \frac{89}{400} W$}
	\State {Let~$\bar v$ be a vertex such that~$G[Y \cup \{\bar v\}]$ and $G[V \setminus (Y \cup \{\bar v\})]$ are connected.}
	\State {$Y \gets Y \cup \{\bar v\}$}
	\EndWhile
	\State {\textbf{return} \textsc{Balance}($G - Y, w$) $\cup~Y$}
\EndIf
\EndProcedure
\end{algorithmic}
\caption{$\maxminBCP{3}$ approximation algorithm.}
\label{alg:maxmin}
\end{algorithm}


==> Algorithms/min-max4-alg.tex <==
%!TEX root = ../BCP.tex
\begin{algorithm}[H]
\hspace*{\algorithmicindent} \textbf{Input:} vertex-weighted graph $(G,w)$\\
% An instance~$(G, w)$ of~$\minmaxBCP{4}$.\\
\hspace*{\algorithmicindent} \textbf{Output:} a connected~$4$-partition of~$G$.\\
\hspace*{\algorithmicindent} \textbf{Subroutine:} The algorithm~\textsc{Balance}~by Chleb{\'i}kov{\'a}~\cite{Chl96} for~$\minmaxBCP{2}$. 
\begin{algorithmic}[1]
\Procedure {Min-Max-BCP4}{$G, w$}

\State $\{V_1, V_2, V_3\}$ $\gets$ \textsc{Min-Max-BCP3}$(G,w)$
% \While {$w(V_3) > \frac{W}{2}$}
% 	\If {$V_1$ is adjacent to~$V_2$}
% 		\State {$P \gets \textsc{Merge}(V_1, V_2)$}
% 	\ElsIf {$\exists i \in \{1, 2\}$ and $U \subset V_3$ such that $U$ is adjacent to $V_i$, $G[U]$ and $G[V_3 \setminus U]$ are connected and $w(U) + w(V_i) < w(V_3)$}
% 		\State {$P \gets \textsc{Pull}(U, V_i)$}
% 	\Else 
% 		\State {Let~$u \in V_3$ be an~$l$-cut vertex of~$G$.}
% 		\State {Let~$C_1, \ldots, C_{l - 2}$ be the connected components of~$G[V_3] \setminus u$.}
% 		\State {\textbf{return} $\{\{u\} \cup (\bigcup_{i \in [l - 2]} C_i), V_1, V_2\}$}
% 	\EndIf
% \EndWhile

\If {$w(V_3)\leq \frac{1}{2}W$}\label{line:If:half:W}
	\State {$\{V^-_3, V^+_3\}$ $\gets$ \textsc{Balance}$(G[V_3],w)$}  \algorithmiccomment{Assume $w(V^-_3)\leq w(V^+_3)$.}
	\If {$w(V_2) \leq \frac{2}{5} W$} 
		% \State {$\{V_3^-, V_3^+\} \gets \textsc{Balance}(V_3, w)$}
		\State {\Return $\{V_1, V_2, V_3^-, V_3^+\}$} \label{line:return:case1}
	\Else %w(V_2) > \frac{2}{5} W
		\State {Let~$j \in \{2, 3\}$ be such that~$V_1$ is adjacent to~$V_j$, and let~$i \in \{2,3\}\setminus \{j\}$}
		\State {$\{X^-, X^+\} \gets \textsc{Balance}(G[V_1 \cup V_j], w)$} \algorithmiccomment{Assume $w(X^-)\leq w(X^+)$.}
		\State {$\{Y^-, Y^+\} \gets \textsc{Balance}(G[V_i], w)$} \algorithmiccomment{Assume $w(Y^-)\leq w(Y^+)$.}
		\State {\Return $\{X^-, X^+, Y^-, Y^+\}$} \label{line:return:case2}
	\EndIf
\Else
	\State {Let~$u$ be a cut-vertex of $G$ as in Lemma~\ref{lemma:ratio:minmax3}, and let $\mathcal{C}$ be the set of components of $G-u$} \algorithmiccomment{Note that $|\mathcal{C}|\geq 2$ since $\{G[V_1], G[V_2]\} \subseteq \mathcal{C}$.}
	\If{$|\mathcal{C}|=2$}
		\State{Let $v$ be a non-cut vertex of $G[V_2]$}
		\State{\Return{$\{\{u\}, \{v\}, V_1, (V_2\setminus\{v\})\}$}} \label{line:return:case3}
	\Else
		% \State{Let $C^* \in \arg \max_{C \in \mathcal{C}\setminus\{G[V_1], G[V_2]\}} w(C)$}
		\State{Let $C^* \in \mathcal{C}\setminus\{G[V_1], G[V_2]\}$ such that $w(C^*)$ is maximum}	
		\State{Let $X = \bigcup_{C \in \mathcal{C}\setminus\{G[V_1], G[V_2], C^*\}} V(C)$} \algorithmiccomment{It is possible that $X=\emptyset$}
		\State{\Return{$\{\{u\}\cup X, V(C^*), V_1, V_2\}$}} \label{line:return:case4}
	\EndIf
\EndIf
\EndProcedure
\end{algorithmic}
\caption{\textsc{Min-Max-BCP4}}
\label{alg:minmax4}
\end{algorithm}

